Are Visual Explanations Useful? A Case Study in Model-in-the-Loop Prediction

We present a randomized controlled trial for a model-in-the-loop regression task, with the goal of measuring the extent to which (1) good explanations of model predictions increase human accuracy, and (2) faulty explanations decrease human trust in the model. We study explanations based on visual saliency in an image-based age prediction task for which humans and learned models are individually capable but not highly proficient and frequently disagree. Our experimental design separates model quality from explanation quality, and makes it possible to compare treatments involving a variety of explanations of varying levels of quality. We find that presenting model predictions improves human accuracy. However, visual explanations of various kinds fail to significantly alter human accuracy or trust in the model - regardless of whether explanations characterize an accurate model, an inaccurate one, or are generated randomly and independently of the input image. These findings suggest the need for greater evaluation of explanations in downstream decision making tasks, better design-based tools for presenting explanations to users, and better approaches for generating explanations.

==> Neurips 2020 - Age Prediction RCT/experimental_design.tex <==

\section{Experimental Design}
\label{sec:exp_setup}

\subsection{Task}

We study a model-in-the-loop scenario, where participants are shown an input and a model's prediction, and then asked to make their own guess. Our study examines the age prediction task, where users guess a person's age given an image of their face. We chose this task because (a) both models and humans can perform the task with some proficiency, but with far from perfect accuracy, and (b) it is representative of high-stakes real-world scenarios that use similar models in passport recognition and law enforcement \cite{schuba2020facerecog, passport2020}. A discussion of the ethical concerns of tasks that involve predicting demographic features can be found in the Broader Impact section.

\begin{figure}[!ht]
    \begin{subfigure}[b]{.49\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/app/rct_guide_mod}
      \caption{Description of the model and guidelines for interpreting and using the explanations.}
      \label{fig:app-aiguide}
    \end{subfigure}
    \hspace{0.04\textwidth}
    \begin{subfigure}[b]{.5\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/app/rct_guess_mod2}  
      \caption{Users are asked to guess a person's age.}
    \end{subfigure}
    \newline
    % \vspace{-1.5\baselineskip}
\caption{Webapp used to run the human study. Elements boxed in orange are shown or not shown depending on the treatment arm. The model prediction is shown in all cases except the control, and in additional treatments discussed in the Appendix. The saliency map in (b) is shown in the Explanation-based treatments. The description of the model performance in (a) is shown in all treatments involving the model, except for two additional treatments discussed in the Appendix.
}
\label{fig:app}
\end{figure}



% TODO: real life analogue / would not simply defer to one.... 
Users are shown images from the validation and test of the APPA-REAL  dataset \cite{agustsson2017appareal}, which contains 7,591 images with real age labels. We sample images uniformly across ages, and many images are seen by multiple users. We also balance the dataset shown to users by combining equal proportions of images for which the model is more accurate than previously collected human guesses (available in the APPA-REAL data), and vice versa. This allows us to have greater coverage over the more interesting decision space in which the human and model disagree.
The model in our model-in-the-loop task is a Wide Resnet \cite{zagoruyko2016wide} pre-trained on the IMDB-WIKI dataset \cite{rothe2015dex} and fine-tuned on the APPA-REAL dataset. Trained to predict the real ages, this model gets near human-performance with a 5.24 mean absolute error (MAE) on the test set of APPA-REAL, and is more accurate than the previously collected guesses 46.9\% of the time. We call this the ``strong'' model.

% Users are shown images from the validation and test set of the APPA-REAL dataset. Images are sampled uniformly across ages, and many images are seen by multiple users. We also partitioned the images we show users into two subsets: images in which the model is more accurate than the apparent age label, and vice versa. We keep only images in which the model prediction and the apparent age differ by at least 3 years, and each user is shown 5 images from each subset. This allows us to have greater coverage over the more interesting decision space in which the human and model disagree.
% % We call these the \textit{Model-Is-Useful} and \textit{Model-Not-Useful} subsets. 


% \jda{I would organize this paragraph as ``here's the data we show to the users; here's the model we use for model-in-the-loop decisions''.}
% \jda{There is no ``weak'' model in the body of the paper anymore, so can we call this the ``true'' model rather than the ``strong'' model?}
% We use a Wide Resnet \cite{zagoruyko2016wide} pre-trained on the IMDB-WIKI dataset \cite{rothe2015dex} and fine-tuned on the APPA-REAL dataset \cite{agustsson2017appareal}, which contains real age and ``apparent'' age labels for 7,591 images. Apparent ages were crowdsourced on an online platform. Trained to predict the real ages, this model gets near human-performance with a 5.24 mean absolute error (MAE) on the test set of APPA-REAL, and is more accurate than the apparent age labels 46.9\% of the time. We call this the ``strong'' model.
% \jda{Still think you need to unpack ``apparent'' age more: can you just call it ``a previous round of human predictions''? Does it need to be mentioned at all---why not compare to your own no-model-pred number?}


\subsection{Treatments}
Users are randomly placed into different experimental conditions, or treatment arms, allowing us to measure the effect of specific interventions. Different treatments vary aspects of the human-AI system, such as whether the model prediction is shown and what kind of explanation accompanies it. Elements of the experiment are shown in Figure \ref{fig:app}, including how model predictions is presented to the participants. The full set of treatments are listed in Table \ref{tab:supp-treatments}. Our main experiments focus on the effect of showing explanations of varying quality alongside model predictions. Additional experiments further exploring showing explanations alone, and the effect of the description of the model performance, are described in the Appendix.

\paragraph{Baseline treatments}
Our two main baselines are (a) the \textit{Control} treatment, in which the user guesses without the help of the model, and (b) the \textit{Prediction} treatment, in which the user guesses with the model prediction shown but without an explanation shown.

\paragraph{Explanation-based treatments}
These treatments show explanations in addition to the model prediction. Our explanations are pixel-wise importances, or saliency maps, calculated using integrated gradients \cite{sundararajan2017axiomatic}. For each pixel, we sum the absolute value of the channel-wise attributions, then normalize these pixel attribution scores by the 98th percentile of scores across that image. Users are given a guide for how to interpret the saliency maps (Figure \ref{fig:app-aiguide}) and also explicitly asked to consider the explanation when making their own guess. 
% Our survey results indicate

Explanations of varying quality are shown in Figure \ref{fig:img-atts}. In addition to the strong explanations, we also tested two versions of lower quality saliency maps. Importantly, these varying explanations are all shown with predictions from the same strong model, which isolates the effect of the explanation.

\begin{itemize}[topsep=0pt, itemsep=0ex]
    \item \textit{Explain-strong}. These are saliency maps from the same model whose predictions are shown to users. These explanations tend to focus on, in decreasing order, (a) the areas around the eyes, (b) lines anywhere on the face, and (c) regions around the mouth and nose.
    % \jda{as above---rather than ``strong model'', ''the same model whose predictions are shown to users''}
    \item \textit{Explain-spurious}. We train a ``spurious'' model by modifying the APPA-REAL dataset to contain spurious correlations between the background and the label. The area outside the face bounding box is modified by scaling the pixel values by $\alpha$, which is a linear mapping $f(age)$ from the [0,100] age range to a value in [0.25, 5.0]. Saliency maps from the spurious model often focus on both the face and the background. As with all explanation-based treatments, we show the spurious model's saliency map with the predictions from the strong model.
    % \jda{clarify that you show IG salience maps from the spurious model in conjunction with predictions from the real model}
    \item \textit{Explain-random}. We also test completely uninformative, input-agnostic saliency maps that do not focus on the face. To generate these attributions, we first sample an anchor point around the border of the image. We then sample 50 points in a window around the anchor point, which are used as the centers for 2D Gaussians that we then combine. These are similarly normalized and mapped to the same colorscale as the integrated gradients attributions.
\end{itemize}

``Algorithmic aversion'' refers to human loss of trust in a model after seeing it make a mistake \cite{dietvorst2015algorithm, yin2019understanding}. Our question is whether faulty explanations could act as a similar deterrent. A model may be accurate overall but still have undesired behavior. Explanations could expose those deficiencies and serve as a nudge to not trust the model.
% In a real-world scenario, a model may be accurate overall but have biased or undesired behavior. 

\paragraph{Design-based treatments}
We also compare against existing and novel design-based treatments, which vary the description of the model and the way the model's predictions are shown. We are interested in whether these simple framing approaches can be as effective at increasing accuracy or trust as explanation-based treatments. The \textit{Delayed Prediction} treatment tests the effect of anchoring bias \cite{kahneman1982judgment} and was previously shown to work well for improving accuracy in \cite{green2019principles}. We record the initial guess, show the model prediction, then ask for a final guess. The \textit{Empathetic} treatment personifies the model as an AI named Pat, shown in Figure \ref{fig:pat} in the appendix. When a human perceives a computer to be more similar to themselves, they may be more cooperative and find information from the computer to be of higher quality \cite{nass1996can}. We state ``Like every teammate, Pat isn't perfect'' and show Pat next to every prediction. The \textit{Show Top-3 Range} treatment tests a form of uncertainty by showing the range of the models's top 3 predicted ages. The user is told ``The AI's guess will be shown as a range, e.g. 27-29. Sometimes the range may be wider, e.g. 27-35. When the range is wider, this means the AI is more uncertain about its guess.''

% We cross the lower quality saliency map treatments with not stating the model's performance, with the hypothesis.... that faulty explanations would have a larger effect if the user is not told the model has near-human performance. 

% that important regions are: ``(1) the areas around the eyes, and (2) lines anywhere on the face. The next two most important regions are around the mouth and nose.'' The researchers manually went through 200 saliency maps and tallied regions in red in order to determine these features. Users are reminded of these guidelines at every image. This last approach is similar in spirit to \cite{lai2020chicago}.


\subsection{Metrics} 

We measure and analyze four quantities: (1) the \textbf{error} of the user's guess (the absolute value of the difference between the guess and the \emph{ground-truth} age label), (2) \textbf{trust} (quantified as the absolute value of the difference between the guess and the \emph{model's} prediction), (3) the time
spent making the guess, and (4) answers to post-survey questions on how the model prediction was used in their decision-making process and how reasonable the explanations seemed. Our definition of trust follows previous work operationalizing trust as \textit{agreement} with model predictions \cite{yin2019understanding, zhang2020effect, lai2019human}.
% \eric{mention briefly why we measure trust this way / why human self-evaluations are unreliable? Cite}

% R=-0.18, p=7.4e-08


% \begin{enumerate}[topsep=0pt, itemsep=0ex]
%     \item How capable does the AI model seem? (1-7 Likert scale)
%     \item How did you use the model's prediction in your decision-making process? (Freeform)
%     \item How easy to understand were the AI's explanations? Did the explanations seem reasonable? (1-7 Likert scale)
%     % \item What did you learn from the AI's explanations? (Freeform)
% \end{enumerate}


We use a mixed-effects regression model to estimate error and trust as defined above. The model includes fixed-effect terms $\beta_{\textrm{image\_age}}$, the age of the person in the image (which is correlated with the absolute error, $\rho=0.21$, $p < 2.2e^{-16}$), and $\beta_{\textrm{treatment}}$, for each of the treatments. We also include random-effect intercept terms $z_{\textrm{user}}$ and $z_{\textrm{image}}$ to capture effects specific to each image and user. The model is defined as follows, where $\langle$target$\rangle$ is the error or trust defined above.
\begin{equation}
    \label{eq:reg}
    y_{\textrm{$\langle$target$\rangle$}} = \beta_{0} + 
    \beta_{\textrm{treatment}} \cdot x_{\textrm{treatment}} +
    \beta_{\textrm{image\_age}} \cdot x_{\textrm{image\_age}} +
    z_{\textrm{user}} \cdot x_{\textrm{user}} + 
    z_{\textrm{image}} \cdot x_{\textrm{image}} +
    \epsilon
\end{equation}


% which has a statistically significant correlation with the error.

\subsection{Experiment Details}
We ran experiments on Amazon Mechanical Turk, with 1,058 participants.
Participants were incentivized to perform well on the task by paying top performers a 100\% bonus.
Prior to data collection, we conducted a two-tailed power analysis using the mean and standard deviation of previously collected guesses in the APPA-REAL dataset. In order to detect 1 year differences between treatments, we needed to collect 546 guesses per treatment. We ultimately collected 827.5 guesses (82.75 participants) per treatment, 
which would allow us to detect a 1 year difference of means at the p < 0.05 level with probability 93\%.
% With 827 guesses per treatment, we would detect a 1-year difference of means at the p<0.05 level with probability x

% There were 1,058 participants, with an average of 82.75 participants (827.5 guesses) per treatment.
%  

% https://www.stat.ubc.ca/~rollin/stats/ssize/n2.htwo 
% mu1: 7.154
% mu2: 6.154
% sigma: 5.897

% \subsection{Experiment 1: Improving Accuracy} 

% We state the model performance by ``Overall, across many images, the AI is roughly on par with human performance. However, this accurary varies for each image. For some images, humans are more accurate than the AI. For others, the AI is more accurate than humans.'' For two of the treatments, this description is not shown. A summary of the arms are shown in Table \ref{tab:arms}, with a more detailed description of certain arms below. 


% \paragraph{Hypotheses.} We had the following hypotheses:
% % Say things in terms of 1) accuracy, 2) timespent, 3) trust?
% \begin{itemize}[topsep=0pt, itemsep=0ex]
%     \item H1.A Showing the model prediction will increase accuracy. The variations (\textit{Design}-based treatments and adding explanations) will further increase accuracy.
%     \item H1.B Explanations alone will increase accuracy but have a small effect.
% \end{itemize}


    % \item \textbf{Delay Model Pred}: This arm tests the effect of anchoring bias \cite{kahneman1982judgment}. We record the initial guess, show the model prediction, then ask for a final guess. This was used previously to measure trust in \cite{yin2019understanding,zhang2020effect}, and was shown to work well for improving accuracy in \cite{green2019principles}.

    % \item \textbf{Explanations alone.} We also tested the effect of explanations alone. The ``Explain-strong, No Pred'' and ``Explain-weak, No Pred'' arms show the saliency maps from the strong and weak model without the prediction. We also test a global, model-level explanation in the ``Explain-guide, No Pred'' condition. Before the task begins, users are shown a grid of saliency maps and told that important regions are: ``(1) the areas around the eyes, and (2) lines anywhere on the face. The next two most important regions are around the mouth and nose.'' The researchers manually went through 200 saliency maps and tallied regions in red in order to determine these features. Users are reminded of these guidelines at every image. This last approach is similar in spirit to \cite{lai2020chicago}.

% \paragraph{Experiment 2: Certification using Explanations.} 
% \subsection{Experiment 2: Certification using Explanations.} 


% \paragraph{Hypotheses.} We had the following hypotheses:
% % Say things in terms of 1) accuracy, 2) timespent, 3) trust?
% \begin{itemize}[topsep=0pt, itemsep=0ex]
%     \item H2.A Faulty explanations (random explanations and explanations from the spurious model) will decrease trust.
%     \item H2.B When the model performance is not stated, random explanations and explanations from the spurious model will decrease trust by a larger amount.
% \end{itemize}



% \paragraph{Hypotheses.} We had the following hypotheses:
% % Say things in terms of 1) accuracy, 2) timespent, 3) trust?
% \begin{itemize}[topsep=0pt, itemsep=0ex]
%     \item H1.A Showing the model prediction will increase accuracy. The variations (\textit{Design}-based treatments and adding explanations) will further increase accuracy.
%     \item H1.B Explanations alone will increase accuracy but have a small effect.
%     \item H2.A Faulty explanations (random explanations and explanations from the spurious model) will decrease trust.
%     \item H2.B When the model performance is not stated, random explanations and explanations from the spurious model will decrease trust by a larger amount.
% \end{itemize}

% \paragraph{Setup and Participants} 
% The experiments were ran on Amazon Mechanical Turk. Each user was randomly assigned to one of the treatment arms with equal probability. There was an average of 82.75 users (827.5 guesses) per treatment arm. 40.3\% of the participants were female, with a mean age of 36.5 (std 10.8).


% We computed pixel-wise importances, or saliency maps, using integrated gradients \cite{sundararajan2017axiomatic}. For each pixel, we sum the absolute value of the channel-wise attributions. We normalize these pixel attribution scores by the 98th percentile of scores across that image. These values are mapped to the JET colormap in the opencv package \cite{opencv_library}. More important regions are red and orange; less important regions are blue and purple. Examples for the strong and weak model are shown in columns 2 and 3 of Figure \ref{fig:img-atts}. Saliency maps from the weak model are often more diffuse.


% \subsection{Models, Explanations, and Data}

% \paragraph{Model} 
% We use a Wide Resnet \cite{zagoruyko2016wide} trained on the APPA-REAL dataset \cite{agustsson2017appareal}, which contains real ages and ``apparent'' ages for 7,591 images. Apparent ages were collected by crowdsourcing guesses on an online platform. Our primary model is also pre-trained on the IMDB-WIKI dataset, which contains 524,230 images with age labels \cite{rothe2015dex}. This model gets near human-performance with a 5.2430 mean absolute error (MAE) on the test set of APPA-REAL, and is better than the crowdsourced guesses 46.9\% of the time. We call this the ``strong'' model. We also test a ``weak'' model in one treatment, which gets 6.8597 MAE and is better than the apparent ages 34.7\% of the time.

% % We also test a weaker model in one treatment; trained only on APPA-REAL and stopped before convergence, the ``weak'' model gets 6.8597 MAE and is better than the apparent ages 34.7\% of the time.
% %  with weights from Imagenet pre-training.
% % The performance of these two models are shown in Table \ref{tab:age-models-stats}. % (TODO: did we use Imagenet weights for either of these?)
% % TODO: do I need this table?

% \paragraph{Explanatons}
% We computed pixel-wise importances, or saliency maps, using integrated gradients \cite{sundararajan2017axiomatic}. For each pixel, we sum the absolute value of the channel-wise attributions. We normalize these pixel attribution scores by the 98th percentile of scores across that image and map them to the JET colormap in the opencv package \cite{opencv_library}.

% % These values are mapped to the JET colormap in the opencv package \cite{opencv_library}. More important regions are red and orange; less important regions are blue and purple. Examples for the strong and weak model are shown in columns 2 and 3 of Figure \ref{fig:img-atts}.


% \paragraph{Data} Users are shown images from the validation and test set of the APPA-REAL dataset. Images are sampled uniformly across ages, and many images are seen by multiple users.

% We also partitioned the images we show to users into two subsets: images in which the model prediction is more accurate than the apparent age label (i.e. human guesses), and vice versa. We keep only images in which the model prediction and the apparent age differ by at least 3 years to more closely examine this effect. Each user is shown 10 images, with 5 coming from each subset. We call these the \textit{Model-Is-Useful} and \textit{Model-Not-Useful} subsets. Showing users a mix of these images allows us to have greater coverage over and examine this effect.

% % Importantly, the apparent age labels allow us to investigate the effect of the \textit{utility} of a model prediction. A model prediction is useful not simply if it is accurate, but also if it is \textit{more accurate than the human's guess}. We can assess this latter notion apriori by comparing the predictions to the apparent age labels. We thus partition our data (and analysis) into two subsets: images in which the model prediction is more accurate than the apparent age label (i.e. human guesses), and vice versa. We call these the \textit{Model-Is-Useful} and \textit{Model-Not-Useful} subsets. We keep only images in which the model prediction and the apparent age differ by at least 3 years to more closely examine this effect. Each user is shown 10 images, with 5 coming from each subset. 
% % Due to interface differences, the apparent ages end up differing slightly from the guesses we collect in the control condition, but the corrrelation is high ($\rho=0.92$). 


==> Neurips 2020 - Age Prediction RCT/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> Neurips 2020 - Age Prediction RCT/related_work.tex <==



\section{Related Work}
\label{sec:related}

% \subsection{Principles of explanations?}

% 1. Some on interpretable model side: frameworks

% 2. Others in experiments. 
% \cite{green2019principles} has 1) improved accuracy, 2) reliability, 3) fairness. 

\paragraph{Interpretable machine learning}
% In parallel with increasingly performant ML models have been efforts to understand their behavior through methods that generate explanations for their predictions. Unfortunately, evaluating explanations has so far been difficult and ad-hoc. Approaches have included human assessments of correctness of explanations, attempts to derive insights from explanations, or seeing if explanations help humans predict model behavior, but the field still lacks a consensus for best practices \cite{sundararajan2017axiomatic, ribeiro2016should, chandrasekaran2017takes, narayanan2018humans}.

% One focus of interpretable machine learning has been on formalizing frameworks and desiderata for interpretability \cite{doshi2017towards,lipton2016mythos}. 
There has been a wide range of methods, including instance-level explanations \cite{ribeiro2016should} vs. global explanations based on feature representations across the dataset \cite{bau2017network}, glass-box methods with access to model gradients \cite{sundararajan2017axiomatic,smilkov2017smoothgrad} vs. black box methods \cite{ribeiro2016should,petsiuk2018rise}, and input feature attributions \cite{ribeiro2016should,sundararajan2017axiomatic,smilkov2017smoothgrad,petsiuk2018rise,bau2017network} vs. natural language explanations \cite{hendricks2016generating,lei2016rationalizing} vs. counterfactuals \cite{wachter2017counterfactual}. Input feature attributions has been a common approach, which we use for our experiment.

Evaluating explanations has included human assessments of correctness, attempts to derive insights from explanations, and seeing if explanations help humans predict model behavior \cite{sundararajan2017axiomatic, ribeiro2016should, chandrasekaran2017takes, narayanan2018humans}. Recent work has also suggested that popular interpretability methods exhibit undesirable properties, such as being unreliably and unreasonably sensitive to minor changes in the input \cite{jain2019attention,kindermans2019reliability,feng2019can}.

% Evaluating explanations has so far been difficult and ad-hoc. Approaches have included human assessments of correctness of explanations, attempts to derive insights from explanations, or seeing if explanations help humans predict model behavior, but the field still lacks a consensus for best practices \cite{sundararajan2017axiomatic, ribeiro2016should, chandrasekaran2017takes, narayanan2018humans}. Recent work has also suggested that common explanations exhibit unintuitive behavior. For example, there is evidence that saliency maps are unreliably and unreasonably sensitive to minor changes in the input \cite{jain2019attention,kindermans2019reliability}, perhaps due to fundamental pathologies of deep neural networks \cite{feng2019can}. These raise the question that we attempt to address -- how effective are explanations?



\paragraph{Model-in-the-Loop experiments}

% As machine learning (ML) becomes increasingly prevalent, there is a greater need to study the interaction between humans and ML-driven systems \cite{rahwan2019machine}. 
% Deep neural networks are being explored in human-AI systems for medical diagnosis \cite{beede2020human, cai2019human, sendak2020human}, creative writing \cite{clark2018creative}, negotiation \cite{zhou2019dynamic}, and content moderation \cite{lai2019human}. 
% It is imperative to better understand these hybrid approaches as (a) more non-experts use ML, and (b) the stakes of the application rise. 

% Surveys by Lubars et. al that people are most comfortable with ``machine-in-the-loop'' settings, in which humans receive guidance from ML models but make the final decision \cite{lubars2019ask}. General guidelines for human-AI interaction have been recently proposed, echoing existing HCI research on the importance of transparency in such systems \cite{amershi2019guidelines}.

% % Human-computer interaction research provides some high-level design recommendations. 
% Based on analysis of existing products that use ML, Amershi et. al offer guidelines for human-AI interaction such as ``Make clear what the system can do'' and ``Make it easy to edit, refine, or recover when the AI system is wrong'' \cite{amershi2019guidelines}. Surveys by Lubars et. al on task delegability found that people are most comfortable with ``machine-in-the-loop'' settings, in which humans receive guidance from ML models but make the final decision \cite{lubars2019ask}. These studies indicate directions for ML research; for instance, the need for a system to be clear in its capabilities suggest explanations and uncertainty estimates may be important capabilities. However, they do not investigate modern neural networks and interpretability methods.

%  how much humans would trust or delegate to a ML model for a hundred tasks such as reading bedtime stories to your child or managing your finances.
% TODO: there is more nuance in the machine in the loop paper I think

Previous experiments have mixed results on the effect of explanations. In a deceptive review detection task, explanations alone helped human performance slightly. However, the best setting was simply showing the prediction alone while informing users of the model's accuracy \cite{lai2019human}. Other work has shown feature-wise importances for low-dimensional inputs to both slightly increase \cite{green2019principles} and decrease accuracy \cite{zhang2020effect}. Explanations have also been found to increase trust and understanding \cite{lai2019human, lim2009and}, but can hurt if they too overtly convey the model's limitations \cite{yeomans2019making}. Model complexity was also examined in \cite{poursabzi2018manipulating}, which found that less complex, transparent, linear models did not help users in an apartment price prediction task. In fact, transparency hindered people from detecting model errors, echoing other work on the risk of cognitive overload \cite{abdulcogam, lage2019human}.
% predict apartment prices given features of the rental
% In a deceptive review detection task, explanations alone helped human performance slightly, and when paired with predictions if users were not told the model's accuracy.

% The authors of \cite{green2019principles} found that providing feature-wise scores for predicting financial risk (e.g. home ownership is important) improved predictive accuracy slightly. However, feature-wise importances have also been found to decrease accuracy \cite{zhang2020effect}. Explanations have been shown to increase trust and understanding of the model \cite{lai2019human, lim2009and}, but can also hurt if they too overtly convey limitations of the model \cite{yeomans2019making}.
% In a deceptive review detection task, explanations alone helped human performance (57\% vs. 51\%), and when paired with predictions if users were not told the model's accuracy (72.5\% vs  61.9\%)
% Automated rationale generation RL \cite{ehsan2019automated}.
% Moreover, no joint human-AI setting outperformed the model 

% TODO combine this with above and shorten? Other studies have investigated model and explanation complexity. Less complex, transparent, linear models did not help prediction in the task of predicting apartment prices given features of the rental. In fact, transparency actually hindered people from detecting mistakes by the model \cite{poursabzi2018manipulating}, with cognitive overload as a possible reason \cite{abdulcogam, lage2019human}.
% perhaps due to cognitive overload \cite{poursabzi2018manipulating}. 
% The importance of considering cognitive overload when designing for explanations and human-AI systems was also examined in \cite{abdulcogam, lage2019human}.

We expand upon these prior works, as their limitations include (a) linear, relatively simple, or non-neural models \cite{poursabzi2018manipulating, feng2019can, binns2018s, lage2019human, lai2019human}, (b) small input feature spaces, making explanations simpler \cite{green2019principles, poursabzi2018manipulating, zhang2020effect}, (c) imbalance of task performance between humans and AI, e.g. human performance is 51\% on a binary classification task (near random), vs. 87\% for the model in \cite{lai2019human, lai2020chicago}, (d) no investigation into using explanations for certification (identifying faulty or biased models) \cite{ binns2018s, feng2019can, green2019principles,  lai2020chicago, lai2019human,poursabzi2018manipulating, tan2018investigating, zhang2020effect}.
% (d) possibly under-powered experiments (e.g. nine and four users per treatment arm, respectively, in  \cite{zhang2020effect} and \cite{feng2019can})

% \begin{enumerate}[topsep=0pt, itemsep=0ex]
%     \item Linear, relatively simple, or non-neural models \cite{poursabzi2018manipulating, feng2019can, binns2018s, lage2019human}.
%     \item Small input feature spaces, making explanations simpler \cite{green2019principles, poursabzi2018manipulating, zhang2020effect}.
%     \item Imbalance of task performance between humans and AI (e.g. human performance is 51\% on a binary classification task (near random), vs. 87\% for the model in \cite{lai2019human, lai2020chicago}).
%     \item Possibly under-powered experiments (e.g. nine and four users per treatment arm, respectively, in  \cite{zhang2020effect} and \cite{feng2019can}).
%     \item Little investigation into using explanations for certification (i.e. a faulty explanation as a signal to not trust the model) \cite{ binns2018s, feng2019can, green2019principles,  lai2020chicago, lai2019human,poursabzi2018manipulating, tan2018investigating, zhang2020effect}.
% \end{enumerate}

% TODO: also talk about older (Lam / Lim) research that does look at explanations, but not with modern models and tools.


% \cite{ cai2019effects}.
 

% \cite{lai2019human} asks users to identify deceptive reviews, i.e. those written by people who had never been to the hotel or for monetary compensations. They show that explanations slightly improve human performance (57\% vs. 51\%) and can increase trust (74\% vs. 64.4\%), though not as much just showing the model prediction. TODO: did they do prediction and explanation?

% \cite{zhang2020effect} asks users to predict whether a person's annual income is greater than \$50,000 given attributes such as their age, education, and occupation. They test the effect of 1) showing confidence scores using uncalibrated probabilities in the form of ``The model's prediction is correct N times out of 10 on individuals similar to this one.'', and 2) feature importances using SHAP \cite{lundberg2017unified}. Neither helped improve overall accuracy, and explanations may actually hurt, though the results are not statistically significant.

% \cite{green2019principles} asks users to people to predict whether a person would (e.g. deafult on their loan) given a narrative profile of the person, and additional predictions and explanations. Explanations may help a little bit. 

% \cite{poursabzi2018manipulating} asks people to predict prices of apartments in New York City given eight features of the apartments. The model is a linear regression model, and the experiment varies the complexity of the model (two vs. eight features) and the model transparency (showing weights for each feature or not). They find that less complex, transparent models do not actually help prediction. Moreover, transparency can actually hinder people's abilities to detect when the model has made a sizable mistake. TODO: but their model is like impossible to grok...


\paragraph{Certification with explanations} In an ad recommendation setting, explanations allowed users to detect that models were highly limited \cite{eslami2018communicating}. 
The authors of \cite{ribeiro2016should} found users able to identify the better of two models using their interpretable method with 90\% accuracy. \cite{adebayo2018sanity} introduces ``model parameter randomization'' and ``data randomization'' tests to analyze whether explanations are specific to the model and input. However, there have not been extensive human studies of certification. 
% These methods also focus on model-level certification; our study asks the same question but also looks at instance-level certification 


% Interpretability section on page 4-5 talk about people’s desire for more interpretable and specific explanations. Figure 4 shows examples of vague explanations, Figure 5 more specific ones.
% “A Path to Algorithm Disillusionment: “From “Their robots know me” to “Maybe you are not as smart as I thought you were””
% Surfacing explanations illustrated how flawed some of the systems were (e.g. gets person’s main interests wrong)

%  \cite{amodei2016concrete} the problem of accidents in machine learning systems, defined as unintended and harmful behavior that may emerge from poor design of real-world AI systems.

%  \cite{goodfellow2014explaining}.

% Certifying: ML approaches, with connections to adversarial examples and robustness.
% AI2: Safety and Robustness Certification of Neural Networks with Abstract Interpretation


\paragraph{Design of the human-AI system}
% The efficacy of a human-AI approach can depend greatly on how the model and its predictions are presented. 
% For instance, 
Varying the stated accuracy of the model can greatly increase trust in the model, though this trust will decrease if the observed accuracy is low \cite{yin2019understanding}. There are also potential benefits for displaying uncertainty estimates for each prediction \cite{van2019communicating}, though \cite{zhang2020effect} found no improvement when showing confidence scores in textual form. 
% The design of the hybrid system 
``Design''
covers an even broader category of elements, such as incentives to use a ML-driven tool, level of human agency and interactivity, and the ``unremarkability'' of the system \cite{yang2019unremarkable}. These can often determine success in real-life settings \cite{cai2019human, sendak2020human, cai2019hello, beede2020human}, but are out of the scope of our study.

%  as ``the model's prediction is correct N times out of 10 on individuals similar to this one.''


==> Neurips 2020 - Age Prediction RCT/results_acc.tex <==
\subsection{How do model predictions and explanation quality affect model-in-the-loop accuracy?}

\paragraph{Participants in the Empathetic, Show Top-3 Range, and Explain-strong treatments performed best and outperformed humans without AI.} 

Participants shown the model prediction are more accurate by 2 years on average overall, as seen in Figure \ref{fig:reg-err}. The predictions generally help whenever the human is inaccurate ($\bhu$$\gmo$, $\bhu$$\bmo$), but can hurt when the human is accurate and the model is inaccurate ($\ghu$$\bmo$).

The top-performing treatments have similar effects overall. However, their effects vary in different settings. For example, Show Top-3 Range is potentially more helpful in the $\bhu\gmo$ setting, with a 4.55 improvement in accuracy, and also the only top treatment to not have a statistically significant harmful effect in the $\ghu\bmo$ setting. However, we note that Tukey HSD testing indicates that the pairwise differences between all of these top treatments is not statistically significant.

The results are also a reminder of the importance of the \textit{design} of the human-AI system, with the Empathetic and Show Top-3 Range treatments equally or more effective as our explanation-based treatments.
Understanding these approaches may also help design better explanation-based approaches, as there may be underlying mechanisms that affect both. For example, the Empathetic and Explain-strong treatments both increase trust, and it could be that the former does so through an emotional approach while the latter does so through more logical means.

Improved accuracy is not attributable to the amount of time spent making guesses:
participants in the Control took 5.7 seconds per image, compared to Empathetic (6.4), Explain-strong (5.9), Show Top-3 Range (5.4), and Prediction (5.2).

\begin{figure}[!hbt]
    \centering
    
    \begin{subfigure}{1.0\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/reg_err/plot_reg_err_overall.png}
      \caption{Overall}
      \label{fig:reg-err-overall}
    \end{subfigure}
    \newline
    \begin{subfigure}{.48\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/reg_err/plot_reg_err_hgood-mbad.png}
      \caption{$\ghuman\bmodel$}
      \label{fig:reg-err-hgood-mbad}
    \end{subfigure}
    \hspace{0.02\textwidth}
    \begin{subfigure}{.48\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/reg_err/plot_reg_err_hbad-mgood.png}  
      \caption{$\bhuman\gmodel$}
      \label{fig:reg-err-hbad-mgood}
    \end{subfigure}
    \newline
    
    \caption{Estimates for $y_{error}$ regression. \textbf{Intercept represents control treatment (human alone); other estimates are relative to the intercept. Lower values are better, indicating reduced error}. Bootstrapped 95\% confidence intervals are shown. Starred items are statistically significant, calculated with Bonferroni correction: *p<0.05, **p<0.01, ***p<0.001. Additional treatments and settings are in Appendix Section \ref{sec:supp-results}. While showing the model prediction increased accuracy, the explanation-based treatments did not differ significantly from showing the prediction alone. Pairwise differences between the top treatments were also not statistically significant, in all three settings shown.}
    \label{fig:reg-err}
\end{figure}

\paragraph{The addition of explanations did not improve accuracy.} As seen in Figure \ref{fig:reg-err-overall}, the Explain-strong treatment has a similar effect size to the Prediction treatment. This, along with additional explanation-without-prediction treatments detailed in Appendix Sections \ref{sec:supp-treatments} and \ref{sec:supp-results}, which resulted in small and non statistically significant effects, indicate the limited utility of these explanations for such a visual classification task. Survey responses indicate that participants did indeed examine the highlighted areas and focus on important features such as location-specific wrinkles, but could not extract information that would boost their performance.

It is possible that our results would change if users were extensively trained to interpret and use the saliency maps, instead of only being presented with our short guide.
We do note, however, that prior work on training users to interpret saliency map explanations in a different task did not increase performance when model predictions were also shown \cite{lai2019human, lai2020chicago}. 
% Another reaction is whether the size of the confidence intervals is related to variance in the Mechanical Turk population.
% These are natural questions when considering the implications of our study, but 
We believe nevertheless that one broader takeaway remains the same --- designers of human-AI systems should question the utility of pixel-level saliency explanations when designing ML-powered tools. 


\paragraph{The \textit{quality} of explanations had little effect on accuracy.} Though directionally what one might expect overall (explain-strong < explain-spurious < explain-random), the differences are small and not statistically significant in any setting. This is likely related to how explanation quality had little impact on the \textit{trust} participants placed in the model predictions, discussed in the following section.

==> Neurips 2020 - Age Prediction RCT/results_cert.tex <==
\subsection{How does explanation quality affect human trust and understanding?}

\paragraph{Faulty explanations did not significantly decrease trust in model predictions.} We use the same regression model as in Equation 1 but with ``trust'', the absolute value of the difference between the model's prediction and the user's guess, as the outcome variable. Smaller differences would indicate that explanations can increase the degree to which humans believe model predictions are accurate.
The results are in Figure \ref{fig:reg-trust}.
Strong explanations could \textit{increase} trust up to 1.08 years (CI lower bound) relative to the Prediction treatment (no explanations), while the random explanations could \textit{decrease} trust up to 1.48 years (CI upper bound). These effect sizes could be sizable (30-40\% relative to the intercept mean), but no treatment was statistically significant.
Moreover, the difference between the spurious and random saliency maps is small, and none of the pairwise differences are statistically significant.
These findings hold even when the model prediction is inaccurate ($\bmodel$), indicating
that users are not learning to trust the model based on its predictions alone.
%One hypothesis for these results on the overall data is that faulty explanations are ignored if the model predictions are accurate, but 

These findings, coupled with the large differences in accuracy between the $\ghu\bmo$ and $\bhu\gmo$ settings and the decrease in accuracy in the $\ghu\bmo$ setting (Figure \ref{fig:reg-err}), 
raise the question to what degree humans can identify and ignore erroneous model predictions.
For example, a model that is accurate 98\% of the time but makes large errors in the remaining 2\% can be very dangerous in a high-stakes scenario if humans default to trusting all model predictions. Importantly, these subsets are typically unknown on test sets. Two possible approaches to alleviate this problem are (a) surfacing uncertainty measures as touched upon in the Show Top-3 Range treatment, and (b) training users by showing common model errors on a validation set. We also briefly expand upon the complementarity of human guesses and model decisions in Appendix Section \ref{sec:supp-combine}. 

\begin{figure}[!hbt]
    \centering
    
    \begin{subfigure}{0.68\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/reg_trust/plot_reg_trust_overall.png}
      \caption{Overall}
      \label{fig:reg-trust-overall}
    \end{subfigure}
    \newline
    \begin{subfigure}{.34\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/reg_trust/plot_reg_trust_hgood-mbad.png}
      \caption{$\ghuman\bmodel$}
      \label{fig:reg-trust-hgood-mbad}
    \end{subfigure}
    \hspace{0.0\textwidth}
    \begin{subfigure}{.34\textwidth}
      \centering
      \includegraphics[width=\textwidth, cfbox=lightgray 0.1pt 0.1pt]{imgs/reg_trust/plot_reg_trust_hbad-mgood.png}  
      \caption{$\bhuman\gmodel$}
      \label{fig:reg-trust-hbad-mgood}
    \end{subfigure}
    \newline
    
    \caption{Estimates for $y_{trust}$ regression. \textbf{Intercept represents the Prediction treatment; other estimates are relative to the intercept. Smaller values indicate more trust}, i.e. smaller difference between model prediction and human guess. Bootstrapped 95\% confidence intervals are shown. Starred items are statistically significant, calculated with Bonferroni correction: *p<0.05, **p<0.01, ***p<0.001. Additional stats are in Appendix Section \ref{sec:supp-results}. Pairwise differences between explanation-based treatments were not significant, and faulty explanations did not significnatly decrease trust.}
    \label{fig:reg-trust}
\end{figure}

\paragraph{Most participants claimed that explanations appeared reasonable, \textit{even when they were obviously not focused on faces.}} 
Responses out of 7 to the post-survey question, ``How easy to understand were the AI's explanations? Did the explanations seem reasonable?'', are shown in Figure \ref{fig:att1}. 
Despite the clear flaws in the saliency maps shown in Figure \ref{fig:img-atts}, there were only small differences between the treatments. Participants shown a strong explanation rated the explanations 5.37 / 7, versus 5.05 and 4.71 for the spurious and random explanations. 
% This suggests the possibility that certification within a model-in-the-loop task is difficult and requires more explicit and human-understandable explanations. 
% This suggests the possibility that more explicit, human-understandable explanations are required to decrease trust.
% certification within a model-in-the-loop task is difficult and requires more explicit and human-understandable explanations. 
In the next section, we provide qualitative examples to shed some light into these counterintuitive findings.
% \eric{Mann-Whitney or KS test?}


% \begin{figure}[!hbt]
% \begin{wrapfigure}[14]{R}{0.45\textwidth}
\begin{wrapfigure}{R}{0.4\textwidth}
    \centering
    \includegraphics[width=0.4\textwidth]{imgs/plot_att1.png}
    \caption{Distribution, mean, and 95\% confidence intervals on the intelligiblity of explanations. Response on a 1-7 Likert scale. Participants rated explanations similarly, regardless of the quality of the explanations.}
    \label{fig:att1}
\end{wrapfigure}



==> Neurips 2020 - Age Prediction RCT/supp_for_arxiv.tex <==
% this is just supp.tex but with the usepackage etc. removed

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% EXPERIMENTAL SETUP
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Experimental Setup}

\subsection{Datasets, Models, and Training Details}
\label{sec:supp-models}
The IMDB-WIKI dataset used to pretrain our strong model consists of 524,230 images and age labels, and was partitioned into 90\% train, 5\% validation, and 5\% test splits. The train, validation, and test splits for the APPA-REAL dataset were included in the original dataset\footnote{Download link: \url{http://chalearnlap.cvc.uab.es/dataset/26/data/45/description/}}. We also trained a ``weak'' model for use in one additional treatment, which was not pre-trained on the IMDB-WIKI dataset and not trained until convergence on the APPA-REAL dataset. Saliency maps from the weak model tended to focus on similar features, but were often more diffuse, with fewer red spots. The strong and weak models used pretrained ImageNet weights, while the spurious model was trained from scratch in order to be more tuned to the spurious correlations. The model MAEs are listed in Table \ref{tab:age-models-stats}.

\begin{table}[h]
    \caption{Age prediction model performance in terms of mean absolute error (MAE). The MAE for the Spurious model is on the modified APPA-REAL dataset and has slightly lower MAE than the Strong model precisely because it is tuned into additional spurious correlations.}
    % The last column denotes the percent of images for which the model's prediction was better than crowdsourced guesses (apparent ages).
    \label{tab:age-models-stats}
    \vspace{0.5em}

  \centering
  \begin{tabular}{lcc}
    \toprule
    Model & Valid MAE & Test MAE \\
    \midrule
    Strong & 4.62 & 5.24 \\
    Weak & 5.84 & 6.86 \\
    Spurious & 3.33 & 4.58 \\
    \bottomrule
  \end{tabular}
%   \begin{tabular}{lccc}
%     \toprule
%     Model & Valid MAE & Test MAE & Percent Model Better \\
%     \midrule
%     Strong & 4.6200 & 5.2430 & 46.9 \\
%     Weak & 5.8382 & 6.8597 & 34.7 \\
%     Spurious & 3.3325 & 4.5797 & 51.3 \\
%     \bottomrule
%   \end{tabular}
  
\end{table}

Each model was trained on one GeForce GTX 1080 Ti using Pytorch. We used the Adam optimizer with learning rate 0.001 (after sweeping over [0.01, 0.005, 0.001, 0.0005]). Images were scaled to 224 $\times$ 224. We performed data augmentation during training by applying additive Gaussian noise 12.5\% of the time, Gaussian blur 12.5\% of the time, 20 degree rotations, 5\% scaling and translation operations, horizontal flipping, and hue and saturation adjustments.




\subsection{Treatment Arms}
\label{sec:supp-treatments}

The avatar used for the \textit{Empathetic} treatment is shown in Figure \ref{fig:pat}. The icon was made by Freepik from \url{www.flaticon.com} and can be found at \url{https://www.flaticon.com/free-icon/robot_1587565}.
% \begin{wrapfigure}{r}{0.2\textwidth}
% \begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}[!hbt]
    \centering
    \includegraphics[width=0.1\textwidth]{imgs/pat_the_ai.png}
    \caption{Pat the AI.}
    \label{fig:pat}
\end{figure}
% \end{wrapfigure}

\paragraph{Additional treatments}
We also tested the effect of explanations alone, hypothesizing that they may have a small, but slight effect.
The \textit{Explain-strong, No Pred} and \textit{Explain-weak, No Pred} treatments show the saliency maps from the strong and weak model, respectively, \textit{without the prediction}.

We also tested a global, model-level explanation in the \textit{Explain-guide, No Pred} treatment. Before the task begins, users are shown a grid of saliency maps and told that important regions are: ``(1) the areas around the eyes, and (2) lines anywhere on the face. The next two most important regions are around the mouth and nose.'' The researchers manually went through 200 saliency maps and tallied regions in red in order to determine these features. Users are reminded of these guidelines at every image. This approach is similar in spirit to \cite{lai2020chicago}.

% One such treatment was a model-level explanation, used in the \textit{Explain-guide, No Pred} arm. Before the task begins, users are told the regions of a face the model believes to be most important for predicting age. Users are  reminded of the guidelines but not shown a saliency map at every image. This approach is similar in spirit to the training phases of \cite{lai2020chicago}.

For the faulty saliency maps, we additionally tested not stating the model's performance in the \textit{No Acc} treatments.
% , as shown in Figure \ref{fig:app-aiguide}.
We hypothesized that allowing users to come to their own conclusion about the model's ability would result in the faulty explanations having a larger effect.


\begin{table}[h]

  \caption{Full list of treatment arms. All model predictions are from the same ``strong'' model.}
  \label{tab:supp-treatments}
  \vspace{0.5em}
  
  \centering
  \begin{tabular}{lll}
    \toprule
    & \bf Treatment Arm & \bf Shorthand Description\\
    \toprule
    & Control & Ask for age without help of model \\
    \midrule
    & Prediction & User is shown model's prediction \\
    
    \midrule
    \multirow{3}{*}{\rotatebox[origin=c]{90}{\emph{Design}}}
    & Delayed Prediction & User guesses before and after seeing model's prediction \\
    & Empathetic & Model is described as a fallible ``Pat the AI''  \\
    & Show Top-3 Range & Prediction shown as range of top-3 values, e.g. 28-32 \\

    \midrule
    \multirow{7}{*}{\rotatebox[origin=c]{90}{\emph{Explanations}}}
    % \multirow{3}{*}{\rotatebox[origin=c]{90}{\emph{Explanations}}}
    & Explain-strong & Show strong model's saliency map \\
    & Explain-spurious & Show spurious model's saliency map \\
    \vspace{0.5em}
    & Explain-random & Show random saliency map \\
    & Explain-strong, No Pred & Show strong model's saliency map, hide prediction \\
    & Explain-weak, No Pred & Show weak model's saliency map, hide prediction \\
    \vspace{0.5em}
    & Explain-guide, No Pred & Show summary of feature importances, hide prediction \\
    
    % \midrule
    % \multirow{4}{*}{\rotatebox[origin=c]{90}{\emph{Certification}}}
    & Explain-spurious, No Acc & Show spurious model's saliency map, hide model's accuracy  \\
    & Explain-random, No Acc & Show random saliency map, hide model's accuracy \\
    \bottomrule
  \end{tabular}
  
\end{table}




\subsection{Participant Demographics}
40.3\% of the participants were female, with a mean age of 36.5 (standard deviation 10.8).




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ACCURACY
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Results}
\label{sec:supp-results}

The full regression results for MAE, accuracy, and trust are shown in Tables \ref{tab:supp-mae}, \ref{tab:supp-err-reg}, and \ref{tab:supp-trust-reg}. We briefly cover findings from the additional treatments as follows:

\begin{itemize}
    \item The instance-level explanation-only treatments (\textit{Explain-strong, No Pred and Explain-weak, No Pred}) had small, non-statistically significant effects on accuracy.
    \item The model-level explanation-only treatment, \textit{Explain-guide, No Pred}, was helpful overall (1.2 years increase in accuracy, compared to 1.8 years increase in the \textit{Prediction} treatment). It was also as helpful as the top performing treatments when both humans and models were inaccurate, i.e. in the $\bhuman\bmodel$ setting.
    \item Contrary to our hypothesis, hiding the model performance did not significantly increase or decrease the effect of the faulty explanations. Directionally, however, it appeared to \textit{increase trust} in the $\bhuman\bmodel$ setting. It may be that the statement on model performance actually emphasized the fallability of the model.
\end{itemize}


% \subsection{Accuracy}
% \label{sec:supp-acc}



% explain-weak case: ``I tried to tell why the AI was highlighting areas of the face such as wrinkles but it seemed like it was highlighting basically the same areas on every face so I didn't find it to be that much of a help.'', ``Not much. It seemed to be picking areas at random.''


\begin{table}[!htbp]

    \caption{Mean absolute error of guesses for all treatments. Bootstrapped 95\% confidence intervals in parentheses. 
    % We note that the MAE is higher for the ``Model Alone'' case than the MAE stated in the \ref{sec:exp_setup} section because we sample uniformly across the entire age range, and errors are often much larger when the person is older.
    }
   \label{tab:supp-mae}
   \vspace{0.5em}
   
% \begin{wraptable}{R}{0.4\textwidth}
      \centering
      \begin{tabular}{lc}
        \toprule
        % Treatment Arm & MAE & Lower & Upper \\
        Treatment Arm & MAE \\
        \midrule
        % Paste output below
        Control (Human Alone) & 10.0 (9.4 - 10.5) \\
        Model Alone & 8.5 (8.3 - 8.7) \\
        Prediction & 8.4 (7.8 - 9.0) \\
        \midrule
        Explain-strong & 8.0 (7.5 - 8.5) \\
        Explain-spurious & 8.5 (8.0 - 9.1) \\
        Explain-random & 8.7 (8.1 - 9.2) \\
        \midrule
        Delayed Prediction & 8.5 (8.0 - 9.0) \\
        Empathetic & 8.0 (7.6 - 8.5) \\
        Show Top-3 Range & 8.0 (7.4 - 8.5) \\
        \midrule
        Explain-strong, No Pred & 9.7 (9.2 - 10.3) \\
        Explain-weak, No Pred & 10.2 (9.5 - 10.9) \\
        Explain-guide, No Pred & 9.4 (8.9 - 10.0) \\
        \midrule
        Explain-spurious, No Acc & 8.2 (7.6 - 8.8) \\
        Explain-random, No Acc & 8.0 (7.6 - 8.5) \\
        \bottomrule
      \end{tabular}
% \end{wraptable}
\end{table}


% REGRESSION
\begin{table}
      \caption{Estimates for $y_{error}$ regression. \textbf{Intercept represents control treatment (human alone); other estimates are relative to the intercept. Lower values are better, indicating reduced error}. Bootstrapped 95\% confidence intervals are shown in parentheses; starred items are statistically significant, calculated with Bonferroni correction: *p<0.05, **p<0.01, ***p<0.001.}
      \label{tab:supp-err-reg}
      \vspace{0.5em}
      
      \begin{subtable}{1.0\textwidth}
      
      \centering
      \begin{tabular}{Ll}
      
        \toprule
         & \multicolumn{1}{l}{Overall} \\
        \midrule 
        
        % Paste here
        \beta_{\textrm{intercept}} & \multicolumn{1}{l}{5.9 (4.6,7.2)***}\\
        \midrule
        \beta_{\textrm{prediction}} & \multicolumn{1}{l}{-1.8 (-2.6,-1.1)***}\\
        \midrule
        \beta_{\textrm{delay-model-pred}} & \multicolumn{1}{l}{-2.0 (-2.8,-1.2)***}\\
        \beta_{\textrm{empathetic}} & \multicolumn{1}{l}{-2.2 (-3.0,-1.2)***}\\
        \beta_{\textrm{show-top-3-range}} & \multicolumn{1}{l}{-2.2 (-2.9,-1.3)***}\\
        \midrule
        \beta_{\textrm{explain-strong}} & \multicolumn{1}{l}{-2.2 (-3.2,-1.3)***}\\
        \beta_{\textrm{explain-spurious}} & \multicolumn{1}{l}{-1.9 (-2.7,-1.2)***}\\
        \beta_{\textrm{explain-random}} & \multicolumn{1}{l}{-1.6 (-2.5,-0.9)***}\\
        \midrule
        \beta_{\textrm{explain-strong\_no-pred}} & \multicolumn{1}{l}{-0.5 (-1.5,0.3)}\\
        \beta_{\textrm{explain-weak\_no-pred}} & \multicolumn{1}{l}{0.2 (-0.7,0.9)}\\
        \beta_{\textrm{explain-guide\_no-pred}} & \multicolumn{1}{l}{-1.2 (-2.0,-0.4)*}\\
        \midrule
        \beta_{\textrm{explain-spurious\_no-acc}} & \multicolumn{1}{l}{-1.9 (-2.7,-1.0)***}\\
        \beta_{\textrm{explain-random\_no-acc}} & \multicolumn{1}{l}{-2.0 (-2.6,-1.2)***}\\
        \midrule
        \beta_{\textrm{image-age}} & \multicolumn{1}{l}{0.1 (0.0,0.1)***}\\
        
        % Finish
        \bottomrule
      \end{tabular}
      \caption{Overall}
      \end{subtable}
      
      \begin{subtable}{1.0\textwidth}
      \small
      \centering
      \begin{tabular}{Lllll}
        \toprule
        %  & \multicolumn{1}{l}{$\ghu\gmo$} 
        %  & \multicolumn{1}{l}{$\ghu\bmo$}
        %  & \multicolumn{1}{l}{$\bhu\gmo$} 
        %  & \multicolumn{1}{l}{$\bhu\bmo$} \\
         & \multicolumn{1}{l}{$\ghuman\gmodel$} 
         & \multicolumn{1}{l}{$\ghuman\bmodel$}
         & \multicolumn{1}{l}{$\bhuman\gmodel$} 
         & \multicolumn{1}{l}{$\bhuman\bmodel$} \\
        \midrule 
        N & 4940 & 1802 & 1721 & 2812 \\
        \toprule
         
        \beta_{\textrm{intercept}} & \multicolumn{1}{l}{3.3 (2.9,3.7)***} & \multicolumn{1}{l}{4.2 (3.6,4.8)***} & \multicolumn{1}{l}{13.6 (12.1,14.8)***} & \multicolumn{1}{l}{12.7 (10.3,15.9)***}\\
        \midrule
        \beta_{\textrm{prediction}} & \multicolumn{1}{l}{-0.3 (-0.6,0.0)} & \multicolumn{1}{l}{1.1 (0.5,1.8)**} & \multicolumn{1}{l}{-2.3 (-4.3,-1.1).} & \multicolumn{1}{l}{-2.0 (-3.4,-0.7)*}\\
        \midrule
        \beta_{\textrm{delay-model-pred}} & \multicolumn{1}{l}{-0.1 (-0.4,0.3)} & \multicolumn{1}{l}{0.8 (0.3,1.3).} & \multicolumn{1}{l}{-2.9 (-4.5,-1.3)**} & \multicolumn{1}{l}{-2.3 (-3.5,-1.0)**}\\
        \beta_{\textrm{empathetic}} & \multicolumn{1}{l}{-0.4 (-0.7,-0.0)} & \multicolumn{1}{l}{1.2 (0.6,2.0)**} & \multicolumn{1}{l}{-2.6 (-4.2,-0.9)*} & \multicolumn{1}{l}{-2.7 (-3.7,-1.6)***}\\
        \beta_{\textrm{show-top-3-range}} & \multicolumn{1}{l}{-0.4 (-0.8,-0.0)} & \multicolumn{1}{l}{0.8 (0.3,1.4)} & \multicolumn{1}{l}{-4.5 (-6.4,-2.5)***} & \multicolumn{1}{l}{-1.7 (-2.8,-0.8)*}\\
        \midrule
        \beta_{\textrm{explain-strong}} & \multicolumn{1}{l}{-0.2 (-0.6,0.1)} & \multicolumn{1}{l}{1.1 (0.5,1.6)*} & \multicolumn{1}{l}{-3.2 (-5.4,-1.2)**} & \multicolumn{1}{l}{-2.4 (-3.4,-1.2)**}\\
        \beta_{\textrm{explain-spurious}} & \multicolumn{1}{l}{-0.2 (-0.5,0.1)} & \multicolumn{1}{l}{1.2 (0.7,1.7)**} & \multicolumn{1}{l}{-2.5 (-3.9,-0.9)*} & \multicolumn{1}{l}{-1.5 (-2.8,-0.3)}\\
        \beta_{\textrm{explain-random}} & \multicolumn{1}{l}{-0.2 (-0.5,0.2)} & \multicolumn{1}{l}{0.8 (0.2,1.3)} & \multicolumn{1}{l}{-2.8 (-4.5,-1.1)**} & \multicolumn{1}{l}{-1.7 (-3.0,-0.5).}\\
        \midrule
        \beta_{\textrm{explain-strong\_no-pred}} & \multicolumn{1}{l}{0.4 (0.0,0.9)} & \multicolumn{1}{l}{0.2 (-0.3,0.8)} & \multicolumn{1}{l}{-1.1 (-2.8,0.4)} & \multicolumn{1}{l}{-1.4 (-2.7,0.0)}\\
        \beta_{\textrm{explain-weak\_no-pred}} & \multicolumn{1}{l}{0.1 (-0.3,0.7)} & \multicolumn{1}{l}{-0.1 (-0.8,0.8)} & \multicolumn{1}{l}{1.0 (-0.9,2.4)} & \multicolumn{1}{l}{-0.6 (-1.8,0.9)}\\
        \beta_{\textrm{explain-guide\_no-pred}} & \multicolumn{1}{l}{0.0 (-0.2,0.4)} & \multicolumn{1}{l}{-0.2 (-0.8,0.3)} & \multicolumn{1}{l}{-1.1 (-2.6,0.8)} & \multicolumn{1}{l}{-2.4 (-3.9,-1.1)**}\\
        \midrule
        \beta_{\textrm{explain-spurious\_no-acc}} & \multicolumn{1}{l}{-0.3 (-0.7,0.1)} & \multicolumn{1}{l}{1.1 (0.5,1.9)**} & \multicolumn{1}{l}{-2.3 (-3.7,-0.8)} & \multicolumn{1}{l}{-1.2 (-2.4,0.1)}\\
        \beta_{\textrm{explain-random\_no-acc}} & \multicolumn{1}{l}{-0.2 (-0.5,0.3)} & \multicolumn{1}{l}{1.1 (0.6,1.8)**} & \multicolumn{1}{l}{-3.0 (-4.7,-1.6)**} & \multicolumn{1}{l}{-2.2 (-3.2,-1.1)**}\\
        \midrule
        \beta_{\textrm{image-age}} & \multicolumn{1}{l}{0.0 (0.0,0.0)*} & \multicolumn{1}{l}{-0.0 (-0.0,0.0)} & \multicolumn{1}{l}{0.0 (0.0,0.1)} & \multicolumn{1}{l}{0.1 (0.0,0.1)*}\\
        
        % Finish
        \bottomrule
      \end{tabular}
      \caption{Splits}
      \end{subtable}
\end{table}




% \clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TRUST
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Trust}
% \label{sec:supp-trust}


\begin{table}
      \caption{Estimates for $y_{trust}$ regression. \textbf{Intercept represents Prediction treatment; other estimates are relative to the intercept. Lower values indicate greater trust}. Bootstrapped 95\% confidence intervals are shown in parentheses; starred items are statistically significant, calculated with Bonferroni correction: *p<0.05, **p<0.01, ***p<0.001.}
      \label{tab:supp-trust-reg}
      \vspace{0.5em}
      
      \begin{subtable}{1.0\textwidth}
      \centering
      \begin{tabular}{Ll}
      
        \toprule
         & \multicolumn{1}{l}{Overall} \\
        \midrule 
        
        % Paste here
        \beta_{\textrm{intercept}} & \multicolumn{1}{l}{3.7 (2.5,4.5)***}\\
        \midrule
        \beta_{\textrm{explain-strong}} & \multicolumn{1}{l}{-0.4 (-1.1,0.4)}\\
        \midrule
        \beta_{\textrm{explain-spurious}} & \multicolumn{1}{l}{0.5 (-0.4,1.2)}\\
        \beta_{\textrm{explain-random}} & \multicolumn{1}{l}{0.5 (-0.3,1.5)}\\
        \midrule
        \beta_{\textrm{explain-spurious\_no-acc}} & \multicolumn{1}{l}{0.3 (-0.5,1.0)}\\
        \beta_{\textrm{explain-random\_no-acc}} & \multicolumn{1}{l}{0.4 (-0.5,1.0)}\\
        \midrule
        \beta_{\textrm{image-age}} & \multicolumn{1}{l}{0.0 (0.0,0.0)*}\\
        
        % Finish
        \bottomrule
      \end{tabular}
      \caption{Overall}
      \end{subtable}
      
      \begin{subtable}{1.0\textwidth}
      \centering
      \begin{tabular}{Lllll}
        \toprule
         & \multicolumn{1}{l}{$\ghuman\gmodel$} 
         & \multicolumn{1}{l}{$\ghuman\bmodel$}
         & \multicolumn{1}{l}{$\bhuman\gmodel$} 
         & \multicolumn{1}{l}{$\bhuman\bmodel$} \\
        \midrule 
        N & 4940 & 1802 & 1721 & 2812 \\
        \toprule
         

        \beta_{\textrm{explain-strong}} & \multicolumn{1}{l}{-0.1 (-0.5,0.5)} & \multicolumn{1}{l}{0.1 (-1.1,1.5)} & \multicolumn{1}{l}{-1.1 (-2.7,1.0)} & \multicolumn{1}{l}{0.1 (-1.5,1.6)}\\
        \midrule
        \beta_{\textrm{explain-spurious}} & \multicolumn{1}{l}{0.1 (-0.3,0.7)} & \multicolumn{1}{l}{0.7 (-0.4,1.9)} & \multicolumn{1}{l}{-0.0 (-1.7,1.5)} & \multicolumn{1}{l}{1.0 (-0.3,2.1)}\\
        \beta_{\textrm{explain-random}} & \multicolumn{1}{l}{0.0 (-0.4,0.4)} & \multicolumn{1}{l}{1.0 (0.1,2.4)} & \multicolumn{1}{l}{0.4 (-1.5,2.2)} & \multicolumn{1}{l}{1.4 (-0.2,2.6)}\\
        \midrule
        \beta_{\textrm{explain-spurious\_no-acc}} & \multicolumn{1}{l}{0.3 (-0.1,0.7)} & \multicolumn{1}{l}{0.7 (-0.2,1.9)} & \multicolumn{1}{l}{1.2 (-1.2,3.1)} & \multicolumn{1}{l}{-0.2 (-1.8,1.1)}\\
        \beta_{\textrm{explain-random\_no-acc}} & \multicolumn{1}{l}{0.3 (-0.1,0.8)} & \multicolumn{1}{l}{0.7 (-0.3,1.9)} & \multicolumn{1}{l}{-0.3 (-2.0,1.5)} & \multicolumn{1}{l}{0.2 (-1.2,1.2)}\\
        \midrule
        \beta_{\textrm{image-age}} & \multicolumn{1}{l}{0.0 (-0.0,0.0)} & \multicolumn{1}{l}{0.0 (-0.0,0.1)} & \multicolumn{1}{l}{0.0 (-0.0,0.1)} & \multicolumn{1}{l}{0.0 (-0.0,0.1)}\\
        
        % Finish
        \bottomrule
      \end{tabular}
      \caption{Splits}
      \end{subtable}
      
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% SIMPLE HYBRID MODELS
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage

\section{Additional Analyses}

\subsection{The \textit{economic cost} of Model-in-the-Loop predictions}

We also consider the \textit{economic cost} of a prediction, calculated simply as error $\times$ time. Under this metric, the treatment arms are similar or worse than simply showing the model prediction: Control (56.7), Empathetic (50.6), Explain-strong (47.2), Show Model Pred (43.5), Show Top-3 Range (42.5). We use this simply as an illustrative example, as we believe time and cognitive load are important considerations when designing human-AI systems, especially with possibly complex explanations of high-dimensional inputs.

\subsection{Combining human guesses and model predictions}
\label{sec:supp-combine}

We investigate the possible gain of combining the two predictions in simple hybrid models, whose input features are simply the model's prediction and the human's guess. Such models have been found to outperform either human or machine alone \cite{wang2016deep, phillips2018face}, though this may not always be the case \cite{tan2018investigating}. We perform cross-fold validation and hyperparameter search, with the test MAE results for the top-performing treatments shown in Table \ref{tab:hybrid-models}. 

Follow-up questions to our work include: (a) how the differences between treatments can be related to the complementarity of human and model predictions, and (b) how to best design human-AI systems where the AI complements existing human capabilities.
One experiment could be to derive coarse strategies from these hybrid models, such as important decision tree rules, and test whether these strategies could help further improve accuracy (i.e. ``Trust the model if you think the person is above 60, and the model's prediction is significantly greater than yours.'')
% These can act as sort of a lower-bound / floor for the joint human-AI performance? Or if the combined one doesn't have that much gains, that implies there's more ovlap between human and model? 

\begin{table}[!hbtp]
  \caption{MAE on test split of hybrid models that combine human guesses and model predictions}
  \label{tab:hybrid-models}
  \vspace{0.5em}
  
  \small
  \centering
  \begin{tabular}{lS[round-precision=\precision]S[round-precision=\precision]S[round-precision=\precision]S[round-precision=\precision]}
    \toprule
    & \multicolumn{1}{c}{Prediction} & \multicolumn{1}{c}{Explain-strong} & \multicolumn{1}{c}{Empathetic} & \multicolumn{1}{c}{Show Top-3 Range}\\
    \midrule 
    Human guess (with AI assistance) & 8.3910 & 7.9720 & 7.9894 & 7.9780  \\
    Model prediction & 8.4110 & 8.392 & 8.3181 & 8.5152 \\
    \midrule
    % Logistic Regression & 8.0875 & \bf 7.43 & 9.3780 & 8.3333  \\
    % Decision Tree & 7.1375 & 8.3721 & \bf 5.99 & \bf 6.29  \\
    % Neural Network & \bf 6.28  & 7.5232 & 7.9756 & 7.8000 \\
    Logistic Regression & 8.0875 & 8.3333 & 7.4302 & 9.3780 \\
    Decision Tree & 7.1375 &  6.2933 & 8.3721 & 5.9878 \\
    % 2-layer Neural Net &  6.2750 & 7.8000 & 7.5232 & 7.9756 \\
    % \midrule
    % Mean across hybrid & 7.2 & 7.7 & 7.8 & 7.5 \\
    \bottomrule
  \end{tabular}
\end{table}
% \vspace{-3\baselineskip}



% \clearpage


% \bibliographystyle{plain}
% \bibliography{neurips_2020}

% \end{document}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
